Explainability-Aware One Point Attack for Point Cloud Neural Networks

With the proposition of neural networks for point clouds, deep learning has started to shine in the field of 3D object recognition while researchers have shown an increased interest to investigate the reliability of point cloud networks by adversarial attacks. However, most of the existing studies aim to deceive humans or defense algorithms, while the few that address the operation principles of the models themselves remain flawed in terms of critical point selection. In this work, we propose two adversarial methods: One Point Attack (OPA) and Critical Traversal Attack (CTA), which incorporate the explainability technologies and aim to explore the intrinsic operating principle of point cloud networks and their sensitivity against critical points perturbations. Our results show that popular point cloud networks can be deceived with almost $100\%$ success rate by shifting only one point from the input instance. In addition, we show the interesting impact of different point attribution distributions on the adversarial robustness of point cloud networks. Finally, we discuss how our approaches facilitate the explainability study for point cloud networks. To the best of our knowledge, this is the first point-cloud-based adversarial approach concerning explainability. Our code is available at https://github.com/Explain3D/Exp-One-Point-Atk-PC.

==> notes/Aug16_Note.tex <==
General:
* If this paper get's accepted you could also add the reference to our first paper on Axiv for the camera ready version (this "camera ready version" is the final version after inserting the reviewer comments in case it gets accepted)
☑️* Check if all Link/references to the supplementary material are working.
☑️* Check if all links/references to Figures and Tbls are right in the pdf!

Intro:
☑️replaced for space saving * Reference for LIDAR?

Methods:
☑️* metrix -> matrix
☑️* We detail the stopping .... -> We detail the stopping criteria for OPA and CTA in the next subsection.

Experiments:
☑️* Maybe refer to the code if it also includes all the experiments  or parts of it in the beginning of Sec 4 or whereever it fits in Sec 4 not only in the abstract, you could also use a foot note if this saves space, I would also do this in Paper 1.
4.1
    ☑️* Fig. 4.1 ... 3 examples -> Fig 2 visualizes two/four examples ...?    
4.2
    ☑️* Tbl 2: Maybe also bold for the best results? 
    ☑️* Fig 4.2 -> Fig 3?
    ☑️* maybe write "random, lowest, second-largest" in the text in text/italic format since it is compared in Tbl3
    ☑️* Fig 5: If we have space you might want to add the description of the y and x-aches in the graphs but they are also in the caption, this is is just if we have space

Discussion:
    ☑️* networks(5.2) -> networks (5.2)
    * table 1 presents an .. -> Table 4 presents an ...

Conclusion:
    ☑️* As the first ... -> As the first network attack method incorporating explainability, ...
 
Supplementary:
* Check if everything that is listed here is also referenced in the main Paper. Maybe if you have time write 3 or 4 sentences at the beginning of the supplementary about the content overview/structure. You Can also reverence the code here, of it also includes the experiments from the supplementary material
* Is it possible to move Algorithme 1 & 2 on page 2, if not it is also ok.
7.5.2 
    ☑️* see pdf two times: we temporarily set /beta  ... appropriate beta-> use the formula environment
7.6
    ☑️* Add one or two sentences describing the attack success in Figure S7, since you only describe the table. What can I see in the first an second row, why was the attack successful?? just shortly mention the content of the pic.
    
7.7
    ☑️* Title: More AM results -> Additional Activation Maximization (AM) results
    ☑️* Link to the original AM section in the Main paper


